Multitask Network for Joint Object Detection, Semantic Segmentation and Human Pose Estimation in Vehicle Occupancy Monitoring

In order to ensure safe autonomous driving, precise information about the conditions in and around the vehicle must be available. Accordingly, the monitoring of occupants and objects inside the vehicle is crucial. In the state-of-the-art, single or multiple deep neural networks are used for either object recognition, semantic segmentation, or human pose estimation. In contrast, we propose our Multitask Detection, Segmentation and Pose Estimation Network (MDSP) -- the first multitask network solving all these three tasks jointly in the area of occupancy monitoring. Due to the shared architecture, memory and computing costs can be saved while achieving higher accuracy. Furthermore, our architecture allows a flexible combination of the three mentioned tasks during a simple end-to-end training. We perform comprehensive evaluations on the public datasets SVIRO and TiCaM in order to demonstrate the superior performance.

==> bib_save.tex <==
@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})



@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})

@article{drygala2021background,
  title={Background-Foreground Segmentation for Interior Sensing in Automotive Industry},
  author={Drygala, Claudia and Rottmann, Matthias and Gottschalk, Hanno and Friedrichs, Klaus and Kurbiel, Thomas},
  journal={arXiv preprint arXiv:2109.09410},
  year={2021}
}
@inproceedings{yoon2004vision,
  title={Vision based occupant detection system by monocular 3D surface reconstruction},
  author={Yoon, Jason J and Koch, Carsten and Ellis, Tim J},
  booktitle={Conference on Intelligent Transportation Systems (ITSC)},
  pages={435--440},
  year={2004},
  organization={IEEE}
}
@inproceedings{farmer2003occupant,
  title={Occupant classification system for automotive airbag suppression},
  author={Farmer, Michael E and Jain, Anil K},
  booktitle={Conference on Computer Vision and Pattern Recognition (CVPR)},
  volume={1},
  pages={I--I},
  year={2003},
  organization={IEEE}
}
@article{arbogast2003upper,
  title={Upper extremity fractures in restrained children exposed to passenger airbags},
  author={Arbogast, Kristy B and DeNardo, Matthew B and Xavier, Angela M and Durbin, Dennis R and Winston, Flaura K and Kallan, Michael J},
  journal={SAE transactions},
  pages={540--547},
  year={2003},
  publisher={JSTOR}
}
@article{nichols2005impact,
  title={The impact of a nationwide effort to reduce airbag-related deaths among children: an examination of fatality trends among younger and older age groups},
  author={Nichols, James L and Glassbrenner, Donna and Compton, Richard P},
  journal={Journal of safety research},
  volume={36},
  number={4},
  pages={309--320},
  year={2005},
  publisher={Elsevier}
}
@article{ohn2016looking,
  title={Looking at humans in the age of self-driving and highly automated vehicles},
  author={Ohn-Bar, Eshed and Trivedi, Mohan Manubhai},
  journal={Transactions on Intelligent Vehicles (T-IV)},
  volume={1},
  number={1},
  pages={90--104},
  year={2016},
  publisher={IEEE}
}
@inproceedings{diewald2016rf,
  title={RF-based child occupation detection in the vehicle interior},
  author={Diewald, Andreas R and Landwehr, Jochen and Tatarinov, Dimitri and Cola, Patrick Di Mario and Watgen, Claude and Mica, Catalin and Lu-Dac, Mathieu and Larsen, Peter and Gomez, Oscar and Goniva, Thierry},
  booktitle={International Radar Symposium (IRS)},
  pages={1--4},
  year={2016},
  organization={IEEE}
}
@INPROCEEDINGS{DiasDaCruz2021IV,
  author = {Steve {Dias Da Cruz} and Bertram Taetz and Oliver Wasenm\"uller and Thomas Stifter and Didier Stricker},
  title = {Autoencoder Based Inter-Vehicle Generalization for In-Cabin Occupant Classification},
  booktitle = {Intelligent Vehicles Symposium (IV)},
  year = {2021}
} 
@article{zhang2012convex,
  title={A convex formulation for learning task relationships in multi-task learning},
  author={Zhang, Yu and Yeung, Dit-Yan},
  journal={arXiv preprint arXiv:1203.3536},
  year={2012}
}
@inproceedings{zhang2014facial,
  title={Facial landmark detection by deep multi-task learning},
  author={Zhang, Zhanpeng and Luo, Ping and Loy, Chen Change and Tang, Xiaoou},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={94--108},
  year={2014},
  organization={Springer}
}
@inproceedings{heuer2021multitask,
  title={Multitask-centernet (mcn): Efficient and diverse multitask learning using an anchor free approach},
  author={Heuer, Falk and Mantowsky, Sven and Bukhari, Saqib and Schneider, Georg},
  booktitle={International Conference on Computer Vision (ICCV)},
  pages={997--1005},
  year={2021}
}
@inproceedings{he2017mask,
  title={Mask r-cnn},
  author={He, Kaiming and Gkioxari, Georgia and Doll{\'a}r, Piotr and Girshick, Ross},
  booktitle={International Conference on Computer Vision (ICCV)},
  pages={2961--2969},
  year={2017}
}
@inproceedings{nekrasov2019real,
  title={Real-time joint semantic segmentation and depth estimation using asymmetric annotations},
  author={Nekrasov, Vladimir and Dharmasiri, Thanuja and Spek, Andrew and Drummond, Tom and Shen, Chunhua and Reid, Ian},
  booktitle={International Conference on Robotics and Automation (ICRA)},
  pages={7101--7107},
  year={2019},
  organization={IEEE}
}
@inproceedings{kocabas2018multiposenet,
  title={Multiposenet: Fast multi-person pose estimation using pose residual network},
  author={Kocabas, Muhammed and Karagoz, Salih and Akbas, Emre},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={417--433},
  year={2018}
}
@article{redmon2018yolov3,
  title={Yolov3: An incremental improvement},
  author={Redmon, Joseph and Farhadi, Ali},
  journal={arXiv preprint arXiv:1804.02767},
  year={2018}
}
@article{nekrasov2018light,
  title={Light-weight refinenet for real-time semantic segmentation},
  author={Nekrasov, Vladimir and Shen, Chunhua and Reid, Ian},
  journal={arXiv preprint arXiv:1810.03272},
  year={2018}
}
@article{cao2019openpose,
  title={OpenPose: realtime multi-person 2D pose estimation using Part Affinity Fields},
  author={Cao, Zhe and Hidalgo, Gines and Simon, Tomas and Wei, Shih-En and Sheikh, Yaser},
  journal={Tnsactions on Pattern Analysis and Machine Intelligence (PAMI)},
  volume={43},
  number={1},
  pages={172--186},
  year={2019},
  publisher={IEEE}
}
@inproceedings{mccall2016towards,
  title={Towards a taxonomy of autonomous vehicle handover situations},
  author={McCall, Roderick and McGee, Fintan and Meschtscherjakov, Alexander and Louveton, Nicolas and Engel, Thomas},
  booktitle={International Conference on Automotive User Interfaces and Interactive Vehicular Applications (AutoUI)},
  pages={193--200},
  year={2016}
}
@inproceedings{dalal2005histograms,
  title={Histograms of oriented gradients for human detection},
  author={Dalal, Navneet and Triggs, Bill},
  booktitle={Conference on Computer Vision and Pattern Recognition (CVPR)},
  volume={1},
  pages={886--893},
  year={2005},
  organization={IEEE}
}
@inproceedings{redmon2016you,
  title={You only look once: Unified, real-time object detection},
  author={Redmon, Joseph and Divvala, Santosh and Girshick, Ross and Farhadi, Ali},
  booktitle={Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={779--788},
  year={2016}
}
@inproceedings{redmon2017yolo9000,
  title={YOLO9000: better, faster, stronger},
  author={Redmon, Joseph and Farhadi, Ali},
  booktitle={Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={7263--7271},
  year={2017}
}
@inproceedings{liu2016ssd,
  title={Ssd: Single shot multibox detector},
  author={Liu, Wei and Anguelov, Dragomir and Erhan, Dumitru and Szegedy, Christian and Reed, Scott and Fu, Cheng-Yang and Berg, Alexander C},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={21--37},
  year={2016},
  organization={Springer}
}
@inproceedings{liu2018receptive,
  title={Receptive field block net for accurate and fast object detection},
  author={Liu, Songtao and Huang, Di and others},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={385--400},
  year={2018}
}
@InProceedings{Girshick_2015_ICCV,
author = {Girshick, Ross},
title = {Fast R-CNN},
booktitle = {International Conference on Computer Vision (ICCV)},
year = {2015}
} 
@inproceedings{girshick2014rich,
  title={Rich feature hierarchies for accurate object detection and semantic segmentation},
  author={Girshick, Ross and Donahue, Jeff and Darrell, Trevor and Malik, Jitendra},
  booktitle={Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={580--587},
  year={2014}
}
@article{ren2015faster,
  title={Faster r-cnn: Towards real-time object detection with region proposal networks},
  author={Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
  journal={Advances in Neural Information Processing Systems (NeurIPS)},
  volume={28},
  pages={91--99},
  year={2015}
}
@inproceedings{duan2019centernet,
  title={Centernet: Keypoint triplets for object detection},
  author={Duan, Kaiwen and Bai, Song and Xie, Lingxi and Qi, Honggang and Huang, Qingming and Tian, Qi},
  booktitle={International Conference on Computer Vision (ICCV)},
  pages={6569--6578},
  year={2019}
}
@inproceedings{law2018cornernet,
  title={Cornernet: Detecting objects as paired keypoints},
  author={Law, Hei and Deng, Jia},
  booktitle={European conference on computer vision (ECCV)},
  pages={734--750},
  year={2018}
}
@inproceedings{long2015fully,
  title={Fully Convolutional nZetworks for semantic segmentation},
  author={Long, Jonathan and Shelhamer, Evan and Darrell, Trevor},
  booktitle={Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={3431--3440},
  year={2015}
}
@article{long2017fully,  
    author={Shelhamer, Evan and Long, Jonathan and Darrell, Trevor},  
    journal={Transactions on Pattern Analysis and Machine Intelligence (TPAMI)},   title={Fully Convolutional Networks for Semantic Segmentation},   
    year={2017},  volume={39},  number={4},  pages={640-651}}

@inproceedings{ronneberger2015u,
  title={U-net: Convolutional networks for biomedical image segmentation},
  author={Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas},
  booktitle={International Conference on Medical Image Computing and Computer Assisted Intervention (MICCAI)},
  pages={234--241},
  year={2015},
  organization={Springer}
}
@article{liu2015parsenet,
  title={Parsenet: Looking wider to see better},
  author={Liu, Wei and Rabinovich, Andrew and Berg, Alexander C},
  journal={arXiv preprint arXiv:1506.04579},
  year={2015}
}
@inproceedings{zhen2019learning,
  title={Learning fully dense neural networks for image semantic segmentation},
  author={Zhen, Mingmin and Wang, Jinglu and Zhou, Lei and Fang, Tian and Quan, Long},
  booktitle={AAAI Conference on Artificial Intelligence},
  volume={33},
  pages={9283--9290},
  year={2019}
}
@inproceedings{lin2017refinenet,
  title={Refinenet: Multi-path refinement networks for high-resolution semantic segmentation},
  author={Lin, Guosheng and Milan, Anton and Shen, Chunhua and Reid, Ian},
  booktitle={Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={1925--1934},
  year={2017}
}
@inproceedings{chen2018encoder,
  title={Encoder-decoder with atrous separable convolution for semantic image segmentation},
  author={Chen, Liang-Chieh and Zhu, Yukun and Papandreou, George and Schroff, Florian and Adam, Hartwig},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={801--818},
  year={2018}
}
@InProceedings{Zhao_2017_CVPR,
author = {Zhao, Hengshuang and Shi, Jianping and Qi, Xiaojuan and Wang, Xiaogang and Jia, Jiaya},
title = {Pyramid Scene Parsing Network},
booktitle = {Conference on Computer Vision and Pattern Recognition (CVPR)},
year = {2017}
} 
@inproceedings{yang2017stacked,
  title={Stacked hourglass network for robust facial landmark localisation},
  author={Yang, Jing and Liu, Qingshan and Zhang, Kaihua},
  booktitle={Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={79--87},
  year={2017}
}
@inproceedings{cao2017realtime,
  title={Realtime multi-person 2d pose estimation using part affinity fields},
  author={Cao, Zhe and Simon, Tomas and Wei, Shih-En and Sheikh, Yaser},
  booktitle={Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={7291--7299},
  year={2017}
}
@inproceedings{insafutdinov2016deepercut, 
  title={Deepercut: A deeper, stronger, and faster multi-person pose estimation model},
  author={Insafutdinov, Eldar and Pishchulin, Leonid and Andres, Bjoern and Andriluka, Mykhaylo and Schiele, Bernt},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={34--50},
  year={2016},
  organization={Springer}
}
@article{newell2016associative,
  title={Associative embedding: End-to-end learning for joint detection and grouping},
  author={Newell, Alejandro and Huang, Zhiao and Deng, Jia},
  journal={arXiv preprint arXiv:1611.05424},
  year={2016}
}
@inproceedings{pishchulin2016deepcut,
  title={Deepcut: Joint subset partition and labeling for multi person pose estimation},
  author={Pishchulin, Leonid and Insafutdinov, Eldar and Tang, Siyu and Andres, Bjoern and Andriluka, Mykhaylo and Gehler, Peter V and Schiele, Bernt},
  booktitle={Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={4929--4937},
  year={2016}
}

 @InProceedings{Chen_2018_CVPR,
author = {Chen, Yilun and Wang, Zhicheng and Peng, Yuxiang and Zhang, Zhiqiang and Yu, Gang and Sun, Jian},
title = {Cascaded Pyramid Network for Multi-Person Pose Estimation},
booktitle = {Conference on Computer Vision and Pattern Recognition (CVPR)},
year = {2018}
}
@InProceedings{Papandreou_2017_CVPR,
author = {Papandreou, George and Zhu, Tyler and Kanazawa, Nori and Toshev, Alexander and Tompson, Jonathan and Bregler, Chris and Murphy, Kevin},
title = {Towards Accurate Multi-Person Pose Estimation in the Wild},
booktitle = {Conference on Computer Vision and Pattern Recognition (CVPR)},
year = {2017}
}
@InProceedings{Xiao_2018_ECCV,
author = {Xiao, Bin and Wu, Haiping and Wei, Yichen},
title = {Simple Baselines for Human Pose Estimation and Tracking},
booktitle = {European Conference on Computer Vision (ECCV)},
year = {2018}
} 
@InProceedings{Wang_2020_CVPR_Workshops,
    author = {Wang, Chien-Yao and Liao, Hong-Yuan Mark and Wu, Yueh-Hua and Chen, Ping-Yang and Hsieh, Jun-Wei and Yeh, I-Hau},
    title = {CSPNet: A New Backbone That Can Enhance Learning Capability of CNN},
    booktitle = {Conference on Computer Vision and Pattern Recognition (CVPR) Workshops},
    year = {2020}
} 
@article{bochkovskiy2020yolov4,
      title={YOLOv4: Optimal Speed and Accuracy of Object Detection}, 
      author={Alexey Bochkovskiy and Chien-Yao Wang and Hong-Yuan Mark Liao},
      year={2020},
      journal={arXiv preprint arXiv:2004.10934},
}
@INPROCEEDINGS{5206848,  
    author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Kai Li and Li Fei-Fei},  
    booktitle={Conference on Computer Vision and Pattern Recognition (CVPR)},   title={ImageNet: A large-scale hierarchical image database},  
    year={2009}, 
    pages={248-255},  doi={10.1109/CVPR.2009.5206848}
    }
@INPROCEEDINGS{lwRefinenet,
  author    = {Vladimir Nekrasov and
               Chunhua Shen and
               Ian D. Reid},
  title     = {Light-Weight RefineNet for Real-Time Semantic Segmentation},
  booktitle={The British Machine Vision Conference (BMVC)},
  year      = {2018},
}
@article{osokin2018real,
  title={Real-time 2d multi-person pose estimation on CPU: Lightweight OpenPose},
  author={Osokin, Daniil},
  journal={arXiv preprint arXiv:1811.12004},
  year={2018}
}
@InProceedings{Liu_2019_CVPR,
author = {Liu, Shikun and Johns, Edward and Davison, Andrew J.},
title = {End-To-End Multi-Task Learning With Attention},
booktitle = {Conference on Computer Vision and Pattern Recognition (CVPR)},
year = {2019}
} 
@INPROCEEDINGS{DiasDaCruz2020SVIRO,
  author = {Steve {Dias Da Cruz} and Oliver Wasenm\"uller and Hans-Peter Beise and Thomas Stifter and Didier Stricker},
  title = {SVIRO: Synthetic Vehicle Interior Rear Seat Occupancy Dataset and Benchmark},
  booktitle = {Winter Conference on Applications of Computer Vision (WACV)},
  year = {2020}
} 
@inproceedings{lin2014microsoft,
  title={Microsoft coco: Common objects in context},
  author={Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva and Doll{\'a}r, Piotr and Zitnick, C Lawrence},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={740--755},
  year={2014},
  organization={Springer}
}

@inproceedings{dvornik2017blitznet,
  title={Blitznet: A real-time deep network for scene understanding},
  author={Dvornik, Nikita and Shmelkov, Konstantin and Mairal, Julien and Schmid, Cordelia},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={4154--4162},
  year={2017}
}
@inproceedings{teichmann2018multinet,
  title={Multinet: Real-time joint semantic reasoning for autonomous driving},
  author={Teichmann, Marvin and Weber, Michael and Zoellner, Marius and Cipolla, Roberto and Urtasun, Raquel},
  booktitle={2018 IEEE Intelligent Vehicles Symposium (IV)},
  pages={1013--1020},
  year={2018},
  organization={IEEE}
}
@InProceedings{Papandreou_2018_ECCV,
author = {Papandreou, George and Zhu, Tyler and Chen, Liang-Chieh and Gidaris, Spyros and Tompson, Jonathan and Murphy, Kevin},
title = {PersonLab: Person Pose Estimation and Instance Segmentation with a Bottom-Up, Part-Based, Geometric Embedding Model},
booktitle = {European Conference on Computer Vision (ECCV)},
year = {2018}
} 
@article{ranjan2017hyperface,
  title={Hyperface: A deep multi-task learning framework for face detection, landmark localization, pose estimation, and gender recognition},
  author={Ranjan, Rajeev and Patel, Vishal M and Chellappa, Rama},
  journal={Transactions on Pattern Analysis and Machine Intelligence (TPAMI)},
  volume={41},
  number={1},
  pages={121--135},
  year={2017},
  publisher={IEEE}
}
@inproceedings{kokkinos2017ubernet,
  title={Ubernet: Training a universal convolutional neural network for low-, mid-, and high-level vision using diverse datasets and limited memory},
  author={Kokkinos, Iasonas},
  booktitle={Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={6129--6138},
  year={2017}
}
@inproceedings{misra2016cross,
  title={Cross-stitch networks for multi-task learning},
  author={Misra, Ishan and Shrivastava, Abhinav and Gupta, Abhinav and Hebert, Martial},
  booktitle={Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={3994--4003},
  year={2016}
}
@article{gkioxari2014r,
  title={R-cnns for pose estimation and action detection},
  author={Gkioxari, Georgia and Hariharan, Bharath and Girshick, Ross and Malik, Jitendra},
  journal={arXiv preprint arXiv:1406.5212},
  year={2014}
}
@article{rebuffi2017learning,
  title={Learning multiple visual domains with residual adapters},
  author={Rebuffi, Sylvestre-Alvise and Bilen, Hakan and Vedaldi, Andrea},
  journal={arXiv preprint arXiv:1705.08045},
  year={2017}
}
@article{felzenszwalb2009object,
  title={Object detection with discriminatively trained part-based models},
  author={Felzenszwalb, Pedro F and Girshick, Ross B and McAllester, David and Ramanan, Deva},
  journal={Transactions on Pattern Analysis and Machine Intelligence (TPAMI)},
  volume={32},
  number={9},
  pages={1627--1645},
  year={2009},
  publisher={IEEE}
}
@article{caruana1997multitask,
  title={Multitask learning},
  author={Caruana, Rich},
  journal={Machine learning},
  volume={28},
  number={1},
  pages={41--75},
  year={1997},
  publisher={Springer}
}
@article{krahenbuhl2011efficient,
  title={Efficient inference in fully connected crfs with gaussian edge potentials},
  author={Kr{\"a}henb{\"u}hl, Philipp and Koltun, Vladlen},
  journal={Neural Information Processing Systems (NIPS)},
  volume={24},
  pages={109--117},
  year={2011}
}
@inproceedings{csurka2008simple,
  title={A Simple High Performance Approach to Semantic Segmentation.},
  author={Csurka, Gabriela and Perronnin, Florent},
  booktitle={BMVC},
  pages={1--10},
  year={2008},
  organization={Citeseer}
}
@inproceedings{newell2016stacked,
  title={Stacked hourglass networks for human pose estimation},
  author={Newell, Alejandro and Yang, Kaiyu and Deng, Jia},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={483--499},
  year={2016},
  organization={Springer}
}
@inproceedings{huang2017densely,
  title={Densely connected convolutional networks},
  author={Huang, Gao and Liu, Zhuang and Van Der Maaten, Laurens and Weinberger, Kilian Q},
  booktitle={Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={4700--4708},
  year={2017}
}
@article{kim2019lightweight,
  title={Lightweight driver monitoring system based on multi-task mobilenets},
  author={Kim, Whui and Jung, Woo-Sung and Choi, Hyun Kyun},
  journal={Sensors},
  volume={19},
  number={14},
  pages={3200},
  year={2019},
  publisher={Multidisciplinary Digital Publishing Institute (MDPI)}
}
@article{papakostas2021distracted,
  title={Distracted and drowsy driving modeling using deep physiological representations and multitask learning},
  author={Papakostas, Michalis and Das, Kapotaksha and Abouelenien, Mohamed and Mihalcea, Rada and Burzo, Mihai},
  journal={Applied Sciences},
  volume={11},
  number={1},
  pages={88},
  year={2021},
  publisher={Multidisciplinary Digital Publishing Institute (MDPI)}
}
@inproceedings{guesdon2021dripe,
  title={Dripe: A dataset for human pose estimation in real-world driving settings},
  author={Guesdon, Romain and Crispim-Junior, Carlos and Tougne, Laure},
  booktitle={International Conference on Computer Vision (ICCV)},
  pages={2865--2874},
  year={2021}
}
@inproceedings{cai2020learning,
  title={Learning delicate local representations for multi-person pose estimation},
  author={Cai, Yuanhao and Wang, Zhicheng and Luo, Zhengxiong and Yin, Binyi and Du, Angang and Wang, Haoqian and Zhang, Xiangyu and Zhou, Xinyu and Zhou, Erjin and Sun, Jian},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={455--472},
  year={2020},
  organization={Springer}
}
@article{li2019rethinking,
  title={Rethinking on multi-stage networks for human pose estimation},
  author={Li, Wenbo and Wang, Zhicheng and Yin, Binyi and Peng, Qixiang and Du, Yuming and Xiao, Tianzi and Yu, Gang and Lu, Hongtao and Wei, Yichen and Sun, Jian},
  journal={arXiv preprint arXiv:1901.00148},
  year={2019}
}
@article{russakovsky2015imagenet,
  title={Imagenet large scale visual recognition challenge},
  author={Russakovsky, Olga and Deng, Jia and Su, Hao and Krause, Jonathan and Satheesh, Sanjeev and Ma, Sean and Huang, Zhiheng and Karpathy, Andrej and Khosla, Aditya and Bernstein, Michael and others},
  journal={International Journal of Computer Vision (IJCV)},
  volume={115},
  number={3},
  pages={211--252},
  year={2015},
  publisher={Springer}
}
@article{katrolia2021ticam,
  title={Ticam: A time-of-flight in-car cabin monitoring dataset},
  author={Katrolia, Jigyasa Singh and Mirbach, Bruno and El-Sherif, Ahmed and Feld, Hartmut and Rambach, Jason and Stricker, Didier},
  journal={arXiv preprint arXiv:2103.11719},
  year={2021}
}
@inproceedings{pulgarin2017drivers,
  title={Drivers’ Manoeuvre classification for safe HRI},
  author={Pulgarin, Erwin Jose Lopez and Herrmann, Guido and Leonards, Ute},
  booktitle={Conference Towards Autonomous Robotic Systems (TAROS)},
  pages={475--483},
  year={2017},
  organization={Springer}
}
@article{chen2020driver,
  title={Driver behavior analysis via two-stream deep convolutional neural network},
  author={Chen, Ju-Chin and Lee, Chien-Yi and Huang, Peng-Yu and Lin, Cheng-Rong},
  journal={Applied Sciences},
  volume={10},
  number={6},
  pages={1908},
  year={2020},
  publisher={Multidisciplinary Digital Publishing Institute (MDPI)}
}
@InProceedings{Reiss_2020_CVPR_Workshops,
author = {Reiss, Simon and Roitberg, Alina and Haurilet, Monica and Stiefelhagen, Rainer},
title = {Activity-Aware Attributes for Zero-Shot Driver Behavior Recognition},
booktitle = {Conference on Computer Vision and Pattern Recognition (CVPR) },
year = {2020}
} 
@inproceedings{roitberg2020cnn,
  title={Cnn-based driver activity understanding: Shedding light on deep spatiotemporal representations},
  author={Roitberg, Alina and Haurilet, Monica and Rei{\ss}, Simon and Stiefelhagen, Rainer},
  booktitle={International Conference on Intelligent Transportation Systems (ITSC)},
  pages={1--6},
  year={2020},
  organization={IEEE}
}
@inproceedings{martin2019drive,
  title={Drive\&act: A multi-modal dataset for fine-grained driver behavior recognition in autonomous vehicles},
  author={Martin, Manuel and Roitberg, Alina and Haurilet, Monica and Horne, Matthias and Rei{\ss}, Simon and Voit, Michael and Stiefelhagen, Rainer},
  booktitle={International Conference on Computer Vision (ICCV)},
  pages={2801--2810},
  year={2019}
}
@article{jain2016brain4cars,
  title={Brain4cars: Car that knows before you do via sensory-fusion deep learning architecture},
  author={Jain, Ashesh and Koppula, Hema S and Soh, Shane and Raghavan, Bharad and Singh, Avi and Saxena, Ashutosh},
  journal={arXiv preprint arXiv:1601.00740},
  year={2016}
}
@article{abouelnaga2017real,
  title={Real-time distracted driver posture classification},
  author={Abouelnaga, Yehya and Eraqi, Hesham M and Moustafa, Mohamed N},
  journal={arXiv preprint arXiv:1706.09498},
  year={2017}
}
@article{zhou2020towards,
  title={Towards theoretically understanding why sgd generalizes better than adam in deep learning},
  author={Zhou, Pan and Feng, Jiashi and Ma, Chao and Xiong, Caiming and Hoi, Steven and others},
  journal={arXiv preprint arXiv:2010.05627},
  year={2020}
}































